BundledSLAM: An Accurate Visual SLAM System Using Multiple Cameras

Multi-camera SLAM systems offer a plethora of advantages, primarily stemming from their capacity to amalgamate information from a broader field of view, thereby resulting in heightened robustness and improved localization accuracy. In this research, we present a significant extension and refinement of the state-of-the-art stereo SLAM system, known as ORB-SLAM2, with the objective of attaining even higher precision. To accomplish this objective, we commence by mapping measurements from all cameras onto a virtual camera termed BundledFrame. This virtual camera is meticulously engineered to seamlessly adapt to multi-camera configurations, facilitating the effective fusion of data captured from multiple cameras. Additionally, we harness extrinsic parameters in the bundle adjustment (BA) process to achieve precise trajectory estimation.Furthermore, we conduct an extensive analysis of the role of bundle adjustment (BA) in the context of multi-camera scenarios, delving into its impact on tracking, local mapping, and global optimization. Our experimental evaluation entails comprehensive comparisons between ground truth data and the state-of-the-art SLAM system. To rigorously assess the system's performance, we utilize the EuRoC datasets. The consistent results of our evaluations demonstrate the superior accuracy of our system in comparison to existing approaches.

==> LaTeX/Relatedwork.tex <==
\section{Related Work}
\label{sec:related}
\begin{figure*}[ht] % htbp
\centering
\includegraphics[width=0.8\linewidth, height=3in]{figures/overview.png}
\caption{Our BundledSLAM System Pipeline}
\label{fig:graph}
\end{figure*}
% Early research in multi-camera SLAM primarily concentrated on the field of Structure from Motion (SFM). Pless~\cite{1211520} first delve into the theoretical utilization of multiple camera systems in SFM. He deduce a generalized camera model and epipolar constraints, outlining how to implement multi-camera-based offline SFM for self-driving applications. This marked the inaugural use of a multi-camera system in the SFM.

% Building on this, Frahm et al.~\cite{frahm2004pose} introduce the concept of representing multiple cameras with a virtual camera. They achieve pose estimation for multiple camera systems using this approach, even for systems with non-overlapping fields of view. Sola et al.~\cite{4631502} explore the adaptation of single-camera SLAM algorithms for multi-camera SLAM and develope methods for the online automatic calibration of multi-view SLAM systems.

% Harmat~\cite{7} improve the perspective camera model in PTAM by introducing a generalized polynomial model. He equippe a small drone platform with a pair of ground-facing stereo cameras and another wide-angle camera facing in the opposite direction to assess the performance enhancement of PTAM in indoor environments using multiple cameras. Subsequently, Harmat develope the classical SLAM system MCPTAM \cite{8} based on his improved PTAM work. This SLAM system achieve algorithm convergence without requiring precise scale information, thanks to the use of an omnidirectional vision Taylor model and a spherical coordinate update method. The concept of multiple key frames (MKF) was introduced in this work.

% Tribou \cite{9} also worke on methods involving non-overlapping fields of view to enhance the robustness of drone pose estimation based on PTAM. Harmat's research extended into multi-camera pose estimation. Yang et al. \cite{10} employe a common perspective camera model to achieve robust pose tracking on autonomous micro aerial vehicle (MAV) platforms. They demonstrate the flexibility of configuring the number and orientation of cameras and integrating visual information from various perspectives.

% Furthermore, both \cite{trvomcs} and \cite{svo} extend their approaches for multi-camera systems. They employe two parallel threads for estimating and mapping while minimizing photometric errors.
